Sharp Local Minimax Rates for Goodness-of-Fit Testing in multivariate Binomial and Poisson families and in multinomials

We consider the identity testing problem - or goodness-of-fit testing problem - in multivariate binomial families, multivariate Poisson families and multinomial distributions. Given a known distribution $p$ and $n$ iid samples drawn from an unknown distribution $q$, we investigate how large $\rho>0$ should be to distinguish, with high probability, the case $p=q$ from the case $d(p,q) \geq \rho $, where $d$ denotes a specific distance over probability distributions. We answer this question in the case of a family of different distances: $d(p,q) = \|p-q\|_t$ for $t \in [1,2]$ where $\|\cdot\|_t$ is the entrywise $\ell_t$ norm. Besides being locally minimax-optimal - i.e. characterizing the detection threshold in dependence of the known matrix $p$ - our tests have simple expressions and are easily implementable.

==> contents/poubelle.tex <==
\subsection{Testing in Frobenius Norm}

We now characterize the minimax separation radius associated to the distance $d(P,Q) = \norm{P-Q}_2$.

\hfill

\begin{theorem}%[Optimal rate in $\norm{\cdot}_2$].
\label{ThFrob}
Let $P \in \mathbb{R}^{m \times m}$ be a probability adjacency matrix and let $d(P,Q) = \norm{P-Q}_2$. Then the minimax separation radius $\epsilon^*$ for the testing problem \eqref{Test} satisfies:
$$ \epsilon^* \asymp \sqrt{\frac{\norm{P}_2}{n}} + \frac{1}{n}.$$
\end{theorem}



\hfill

%{\color{blue} [alex: Tu n'as pas defini ce que tu veux dire par minimax number of obs, pour le moment que $R^*$. Aussi, si tu veux passer en mode PAC (i.e. nombre de samples necessaires pour atteindre une certaine precision avec grande proba) en general les gens definissent des temps d'arret, c'est legerement different. Je sais pas si tu auras le temps de tout reecrire pour des temps d'arret. Si au contraire tu fais tout en test a taille de sample fixe vaut mieux parler de distance de separation (quitte a avoir un corollaire qui dit que la distance de separation est plus petite que $\epsilon$ (mais faut bien mettre au clair que tu fais pas un temps d'arret mais que tes considerations sont a sample size fixe).]}

%A test $\psi$ will be called optimal if its risk is $\leq \eta$ when the number of observations satisfies [Mettre le numéro de l'équation]

\noindent We provide a simple optimal and easily implementable test. It is based on the following statistic:
\begin{equation*}
    T_2 = \sum_{1\leq i < j \leq m} \left(\frac{S_{ij}}{k} - p_{ij}\right)\left(\frac{S'_{ij}}{k} - p_{ij}\right).
\end{equation*}

For $C_\eta = \frac{2}{\sqrt{\eta}}\wedge \frac{1}{4}$ an optimal test is defined as:
\begin{align*}
    \psi_2 = \left\{\begin{array}{ll}
         0 & \text{if } \abs{T_2} \leq C_\eta \frac{\norm{P}_2}{n}, \\
         1 & otherwise. 
    \end{array}
    \right.
\end{align*}


\begin{proposition}\label{upper_bound_norm2}
There exists a constant $K > 0$ depending only on $\eta$ such that the test $\psi_2$ has a risk $\leq \eta$, i.e. $R_\epsilon(\psi_2) \leq \eta$, whenever 
$$\epsilon  \geq K \left( \sqrt{\frac{\norm{P}_2}{n}} + \frac{1}{n} \right),$$
\end{proposition}


\subsection{Testing in $\norm{\cdot}_1$}

Here, we sort the $N := \frac{m(m-1)}{2}$ entries $(p_{ij})_{i<j}$ of $P$ in decreasing order: $p_1 \geq \cdots \geq p_N$ where $p_l$ is the $l$-th largest element in the set $(p_{ij})_{i<j}$. ($P$ is symmetric, therefore all the information of $P$ is contained in $(p_{ij})_{i<j}$). For an integer $1 \leq I \leq N$, we denote by $P_{\leq I}$ (resp. $P_{> I}$) the matrix $P$ in which we have set to zero all entries $p_i$, with $ i>I$ (resp. $i \leq I$): 
\begin{align*}
    P_{\leq I} = (p_i\;\mathbb{1}_{\left\{i \leq I\right\}})_{i= 1, \cdots, N}  \;\;\;\;\;\;\;\;\;\; \text{ and } \;\;\;\;\;\;\;\;\;\; P_{> I} = (p_i\;\mathbb{1}_{\left\{i > I\right\}})_{i= 1, \cdots, N}
\end{align*}


We denote by $I$ the smallest integer $\leq N$ such that 
$$\sum_{i>I} p_i^2 \leq \frac{C_{tail}}{n^2}$$
where $C_{tail}$ is an absolute constant depending only on $\eta$. We denote by $A$ the largest integer $\leq I$ such that 
$$ p_A^\frac{4}{3} \sum_{i \leq I} p_i^\frac{2}{3} \geq \frac{l_\eta}{n^2}$$
where $l_\eta = \log(1+4(1-\eta)^2)$.

\hfill \break

We now characterize the minimax separation radius for the testing problem (\ref{Test}) in the case where $d(P,Q) = \norm{P-Q}_1$.\\

\begin{theorem}\label{th_norm1}
Let $d(P,Q) = \norm{P-Q}_1$. Then the minimax separation radius $\epsilon^*$ for the testing problem \eqref{Test} satisfies:
$$ \epsilon^* \asymp \sqrt{\frac{\norm{P_{\leq I}}_\frac{2}{3}}{n}} + \norm{P_{>A}}_1 + \frac{1}{n}.$$
\end{theorem}



\hfill 

We provide a simple optimal and easily implementable test. It is based on the following two statistics:
\begin{align*}
    T_{bulk} &= \sum_{ i \leq A}\;\;\frac{1}{p_i^{2/3}} \left(\frac{S_{ij}}{k} - p_{ij}\right)\left(\frac{S'_{ij}}{k} - p_{ij}\right),\\
    &\\
    T_{tail} &= \sum_{i>A} \frac{S_i + S'_i}{n} - p_i.
\end{align*}
    

We propose the following test:

\begin{align*}
    \;\;\; \psi_1 = \left\{\begin{array}{lllll}
         1 & \text{if } T_{bulk} \geq \frac{C_\eta}{n} \norm{P_{\leq A}}_\frac{2}{3}^{1/3} \\
         &\\
         1 & \text{if } T_{tail} \geq C_\eta\sqrt{\frac{\sum_{i>A} p_i}{n}} \\
         &\\
         0 & otherwise. 
    \end{array}
    \right.
\end{align*}

\hfill

\begin{proposition}\label{upper_bound_norm1}
There exists a constant $K>0$ depending only on $\eta$ such that the test $\psi_1$ has a risk $\leq \eta$, i.e. $R_\epsilon(\psi_1) \leq \eta$, whenever
$$\epsilon \geq K\left( \sqrt{\frac{\norm{P_{\leq I}}_\frac{2}{3}}{n}} + \norm{P_{>A}}_1 + \frac{1}{n}\right)$$
\end{proposition}


\subsection{Intuitions of the phenomena involved}

Our results bring into play two regimes involving very different phenomena. 

\begin{itemize}
    \item On the bulk, the phenomenon is similar to that involved in the gaussian signal detection setting [ref] \al{je pense pas que ce soit une bonne idee de dire ca - car justement ici la variance change sur les coordonnees}. We first recall the setting: We are given one observation $X \sim N(\theta, I_d)$ where $\theta \in \mathbb{R}^d$ and $I_d$ denotes the identity matrix of size $d$ (observing only one observation is not restrictive since if we had $X_1, \cdots, X_n \sim N(\theta, I_d)$, we could define $X = \frac{1}{n} \sum_{i=1}^n X_i \sim N(\theta, \frac{1}{n}I_d)$ and which is a sufficient statistic of $X_1, \cdots, X_n$ for $\theta$). We now consider the testing problem:
    \begin{equation*}
        \mathcal{H}_0 : \theta = 0 \;\;\;\;\; \text{ vs } \;\;\;\;\; \mathcal{H}_1(\rho) : \norm{\theta}_2 \geq \rho 
    \end{equation*}
    In the latter case, the optimal radius is $d^\frac{1}{4}$ and the optimal test is 
    $$ \mathbb{1}\left\{ \norm{X}_2^2 \geq d + c_\eta\right\} ~~~~~~ \text{ or equivalently } ~~~~~~ \mathbb{1}\left\{ \norm{X}_2^2 \geq \widetilde{c_\eta} d\right\}$$
    where $c_\eta >0$ and $\widetilde{c_\eta} >1$ are absolute constants depending only on $\eta$. The test statstic is
    $$ \norm{X}_2^2 = \sum_{i=1}^d (X_i - 0)^2$$
    which is an estimator of
    $$\norm{\theta}_2^2 = \norm{\theta - 0}_2^2 = \sum_{i=1}^d \left(\theta_i - 0\right)^2$$
    and the threshold is just the standard deviation of the test statistic $ \norm{X}_2^2$ under $\mathcal{H}_0$.
    
    In the graph testing problem, the optimal test statistic is a renormalized $\chi^2$, namely:
    $$ \sum_{i\leq A} \frac{1}{p_i^b} \left(\frac{S_i}{k} - p_i\right)\left(\frac{S_i'}{k} - p_i\right) $$
    which is actually equivalent to using
    $$ \sum_{i\leq A} \frac{1}{p_i^b} \left[ \left(\frac{S_i + S_i'}{n} - p_i\right)^2 - \mathbb{E}\left(\left(\frac{S_i + S_i'}{n} - p_i\right)^2\right)\right].$$
    This is an estimator of:
    $$ \sum_{i \leq A} \frac{1}{p_i^b}(q_i - p_i)^2.$$
    To compare the two models, $q$ plays the role of the true unobserved parameter $\theta$ and $p$ the role of $0$. The renormalizing factor $\frac{1}{p_i^b}$ can be interpreted as follows. Suppose the data is drawn from $q$ such that $ \left|p_i - q_i\right| =: \Delta_i$. Then on coordinate $i$, the same difference $\Delta_i$ should be much easier to detect when $p_i$ is small than when $p_i$ is large. Multiplying the contribution  $\left(\frac{S_i}{k} - p_i\right)\left(\frac{S_i'}{k} - p_i\right)$ of coordinate $i$ by $\frac{1}{p_i^b}$ magnifies the discrepancy $\Delta_i$ with high probability when $p_i$ is small. The exponent $b$ allows us to balance the bias and standard deviation of the test statistic.\\
    
    Note that in both settings, the test statistics are based on \textit{the second order moment}. In the gaussian case, the second order moment is an estimator of $\norm{\theta}_2^2$. In the graph case, defining the following notation:
    $$ \norm{v}_{p,b}^2 := \sum_i \frac{1}{p_i^b}v_i^2,$$
    the test statistic $T_{bulk}$ is an estimator of $\norm{(p-q)_{\leq A}}_{p,b}$. In the gaussian case, the estimator $\norm{X}_2^2$ is very relevant since under the null, $X$ concentrates with high probability on a sphere of radius $\sqrt{d}$ and of constant width. Thus, with probability at least $1 - \eta/2$, $\norm{X}_2^2$ only takes values in $[d, d + c_\eta] \subset [d, \widetilde{ c_\eta}d]$. The phenomenon is similar in the graph setting: the analogous test statistic concentrates on a sphere too, with radius upper bounded by the threshold under the null. In brief, the phenomenon involved on the bulk is a non-isotropic \textit{subgaussian phenomenon}, which is not surprising given the central limit theorem. Indeed, we have a family of binomial distributions 
    $$ \begin{pmatrix}Bin(n,p_1)\\ \vdots \\Bin(n,p_A) \end{pmatrix} $$
    with all coordinates mutually independent. The test statistic is based on 
    $$ \begin{pmatrix}\frac{Bin(n,p_1)}{n}\\ \vdots \\\frac{Bin(n,p_A)}{n} \end{pmatrix} \;\;\;\;\;\; \text{ which is converges in distribution to }  \;\;\;\;\;\; \mathcal{N}\left(p, \begin{pmatrix}\frac{p_1(1-p_1)}{n} & \cdots & 0 \\ \dots & & \vdots \\ 0 & \cdots & \frac{p_A(1-p_A)}{n} \end{pmatrix} \right)$$
    when $n$ is large enough. What does ``$n$ large enough'' mean? The definition of the index $A$ provides an answer: it is the value of $n$ allowing 
    $$ p_A^\frac{b}{2} \gtrsim \frac{1}{\sqrt{n}\left(\sum_{i \leq I} p_i^r\right)^\frac{1}{4}}$$
    which suggests defining the bulk as the set of indices such that the subgaussian phenomenon occurs.\\
    
    Note that in both settings, the test statistics is a measure of the \textit{dispersion} of the observation around their mean (second order moment) rather than an estimation of the mean itself (first order moment). We use the second order moment as a detection procedure because it concentrates in much narrower high probability zones than the first order moment. However, using such a procedure requires that we \textit{do observe the second order moment}, i.e. the dispersion of the data around its mean. 
    
    but in a model where the variance is different coordinate-wise and depends on the expectation.
\end{itemize}


\al{Je pense que il faut reecrire... Et peut etre placer juste apres bulk - en divisant les choses bornes sup borne inf. Pour le bulk (a diviser entre borne inf et borne sup):
\begin{itemize}
    \item faire un rappel a des papiers de signal detection mais en moins de detail.
    \item dire que ici la variance change suivant les coordonnes - mais ne pas faire le lien Gaussien
    \item essayer d'expliquer quelle inegalite de Hoelder sera saturee (cf borne inf) -- mais dur a faire
\end{itemize}

Pour le tail (a diviser entre borne inf et borne sup):
\begin{itemize}
    \item expliquer que on est dans un regime tres different du regime Gaussien - car on aura au plus un seul edge allume
    \item expliquer comment les deux tests se combinent
    \item raconter difference avec VV et setting $l_2$
    \item Parler de borne inf
\end{itemize}

}


We show here that the definition of $I$ implies this condition (we recall that $I$ is defined such that $\sum_{i > I} n^2p_i^2 \leq C_{tail}(\eta)$). Fixing any index $i > I$, the probability that, among the $n$ graphs, edge $i$ is observed exactly once or exactly zero times is:
\begin{align*}
    (1-p_i)^n + n p_i(1-p_i)^{n-1} &\leq 1 - n p_i + \frac{n^2}{2} p_i^2 + o(n^2 p_i^2) + n p_i \left[1 - (n-1)p_i + o(np_i)\right]\\
    & = 1 - \frac{n^2}{2} p_i^2 + o(n^2 p_i^2)
\end{align*}
so that the probability of observing edge $i$ at least twice is $1 - \left[1 - \frac{n^2}{2} p_i^2 + o(n^2 p_i^2)\right] \asymp n^2 p_i^2$. Therefore, by union bound, the probability that at least one coordinate is observed twice or more among the $n$ realizations is (up to a constant) upper bounded by:
$$ \sum_{i > I} n^2 p_i^2 \lesssim 2 C_{tail}$$

We can now choose $C_{tail}$ so that this happens with small probability, and define $I$ accordingly.

The reason is that the dispersion (or \textit{second order moment}) is very sensitive to the true distribution $Q$ and allows detecting small differences between $P$ and $Q$. 






$$\norm{p-q}_1 \lesssim \norm{p}_1 + \sqrt{\frac{\norm{q}_1}{n}} + \frac{1}{n},$$ 
using $xy \leq \frac{x^2 + y^2}{2}$, 
Now
\begin{enumerate}
    \item If $\norm{q}_1 \lesssim \norm{p}_1+ \frac{1}{n},$ then on $\{T_1 = 0\} \cap \xi$: 
    $$\norm{p+q}_1 \lesssim \norm{p}_1 + \frac{1}{n}.$$
    \item Else if $\norm{q}_1 \gg \norm{p}_1 + \frac{1}{n}$, thus $\norm{p-q}_1 \geq \frac{\norm{q}_1}{2}$, which implies that
    $$\norm{p-q}_1 \gg \norm{p}_1 + \sqrt{\frac{\norm{q}_1}{n}} + \frac{1}{n},$$ \al{Tous ces $\gg$ et$\gtrsim$ a preciser...}
    so that $\{\psi_1 = 0\} \cap \xi$ cannot hold.
%    $\norm{Q_{>A}}_1^2 \lesssim \frac{\norm{Q_{>A}}_1}{n}$ hence $\norm{Q_{>A}}_1, \lesssim \frac{1}{n}$ which yields $\norm{P_{>A}}_1 \lesssim \frac{1}{n}$. 
\end{enumerate}
Therefore, on $\{\psi_1 = 0\} \cap \xi,$ we have 
$$\norm{(p-q)_{>A}}_1 \lesssim \norm{p_{>A}}_1 + \frac{1}{n}.$$




This proves that 
$$\norm{P_{>A}}_1 \leq \left( 1 + \frac{l_\eta}{C_{tail}}  \right)\norm{P_{\geq I}}_1, \;\;\; \text{  hence  } \;\;\; \norm{P_{>A}}_1 \lesssim \norm{P_{\geq I}}_1$$

Now we prove $\norm{P_{\geq I}}_1 \asymp \norm{P_{>I}}_1 + \frac{1}{n}$ in the case $A < I$. Indeed, in this case we have:

$$ \|P_{>I}\|_1 \leq \|P_{\geq I}\|_1  \leq \|P_{>A}\|_1 $$

$$  p_I^{2b}\sum_{i\leq I} p_i^r < \frac{l_\eta}{n^2}$$

Hence the result.


\ju{
[Pas la peine de lire ça en première lecture]
To do this properly, let $M > 0$ be a constant depending on $p$ such that when 
\begin{equation}\label{constant_poisson_moment_1}
   \mathbb{P}\left(Poi(n\sum_{j=1}^d p_j) > M \right) \leq \frac{\eta}{4} 
\end{equation}
Define a constant $C>0$ such that if $\sum_{j=1}^d q_j >C \sum_{j=1}^d p_j$ then we have:
$$ \mathbb{P}\left(Poi(n\sum q_j) > M\right) \geq 1 - \frac{\eta}{4}$$

Then, if $\sum_{j=1}^d q_j >C \sum_{j=1}^d p_j$, we can reject $H_0$ just by checking that $\sum_{j=1}^d Y_j >M$. }\\


This is nice because, for $\bar p$ defined as in \eqref{def_bar_p}, we have proved both
$$ \begin{cases}\rho_{Poi}(n,p) \leq \lambda \rho_{Mult}(n\lambda, \bar{p}/\lambda)\\
&\\
\rho_{Mult}(n,\bar p) \leq \rho_{Poi}(n,p)\end{cases}$$

Moreover, $\rho_{Poi}(n,p) \asymp \rho_{Bin}(n,p) = \lambda \rho_{Bin}(n\lambda, \frac{p}{\lambda})$, by direct calculation from the expression of $\rho_{Bin}(n,p)$ found in the paper. Therefore, we have:

$$ \begin{cases}\rho_{Poi}(n,p) \leq \lambda \rho_{Mult}(n\lambda, \bar{p}/\lambda)\\
&\\
\rho_{Mult}(n,\bar p) \leq \lambda \rho_{Bin}(n\lambda, \frac{p}{\lambda})\end{cases}$$



###############
Preuve UPPER BOUND TAIL
###############




We proceed by contraposition, by showing that if $T_1$ and $T_2$ accept $\mathcal{H}_0$ with high probability, then necessarily $\norm{\Delta_{>A}}_t \lesssim \rho$.\\




We prove lemma \ref{A_and_1_over_n} later on. Consider the event:
$$\xi = \Big\{ |T_i - \mathbb E[T_i]| \leq 
\frac{2}{\sqrt{\eta}}\sqrt{\mathbb V[T_i]},~~~i\in\{1,2\} \Big\}.$$
Using Chebyshev's inequality and a union bound, the probability of $\xi$ is lower bounded by $1-\eta/2$.\\

\

Note that on the event $\{\psi_2 = 0\} \cap \xi,$ we have $ \norm{\Delta}_2 \lesssim \frac{1}{n}$. Indeed, on this set we have $|T_2| \leq \uc\frac{\|p\|_2}{n}$ by definition. Therefore, on $\xi$:
\begin{align*}
    |\mathbb E[T_2]| - |T_2| & \leq  \frac{2}{\sqrt{\eta}}\sqrt{\mathbb V[T_2]}\\
    \Longrightarrow \;\;\;\; \mathbb{E}[T_2]^2 &\leq \left( \frac{2}{\sqrt{\eta}}\sqrt{\mathbb V[T_2]} + \uc \frac{\|p\|_2}{n}\right)^2 \leq \left( \frac{2}{\sqrt{\eta}}\sqrt{\mathbb V[T_2]} + \uc \frac{C_A}{n^2}\right)^2\\
    \Longrightarrow \;\;\;\; \norm{\Delta}_2^4 & \leq \frac{8}{\eta}\mathbb V[T_2] + 2\uc^2C_A^2\frac{1}{n^4} ~~~~ \text{using} (a+b)^2 \leq 2(a^2+b^2)
\end{align*}
Moreover,
\begin{align*}
    \mathbb{V}[T_2] &\leq \sum_{j>A} \frac{q_j^2}{n^2} + \frac{2}{n}q_j\Delta_j^2 \leq \frac{\norm{q}_2^2}{n^2} + \frac{2}{n}\norm{q}_2\norm{\Delta}_2^2 ~~ \text{ by Cauchy-Schwarz}\\
    &\\
    & = \left(\frac{\norm{q}_2}{n} + \norm{\Delta}_2^2\right)^2- \norm{\Delta}^4 \leq \left(\frac{\norm{p}_2 + \norm{\Delta}_2}{n} + \norm{\Delta}_2^2\right)^2- \norm{\Delta}^4 \\
    &\leq \left(\frac{1}{n^2} +\frac{\norm{\Delta}_2}{n} + \norm{\Delta}_2^2\right)^2- \norm{\Delta}^4 ~~ \text{ by Lemma \ref{A_and_1_over_n}}\\
    & \leq \left(\frac{1}{n} + \norm{\Delta}_2\right)^4- \norm{\Delta}_2^4
\end{align*}
\begin{align*}
    \text{which yields: } ~~ \norm{\Delta}_2^4 &\leq \frac{8}{\eta} \left[\left(\frac{1}{n} + \norm{\Delta}_2\right)^4- \norm{\Delta}_2^4\right]+2\uc^2C_A^2\frac{1}{n^4}
\end{align*}
Letting $C_0>0$ be the smallest constant such that $\forall x> C_0: \left(\frac{8}{\eta}+1\right)x^4 -\frac{8}{\eta}(1 + x)^4 + 2\uc^2C_A^2 \geq 0$, which exists since this polynomial of $x$ tends to $+\infty$ when $x \to +\infty$, we therefore have $n\norm{\Delta}_2 \leq \frac{C_0}{n}$.
\\
For brevity, we write this relation holding on $\{\psi_2 = 0\} \cap \xi:$
\begin{equation}\label{psi2_and_xi}
    \norm{\Delta}_2 \lesssim \frac{1}{n}
\end{equation}


%$\norm{(p-q)_{>A}}_2^2 \lesssim \frac{\norm{p_{>A}}_2}{n} + \frac{1}{n^2}$ which implies by Lemma \ref{A_and_1_over_n},that $$\norm{(p-q)_{>A}}_2^2 \lesssim \frac{1}{n^2}.$$





%Now, if $T_2$ accepts with high probability, then classically, $\norm{(P-Q)_{>A}}_2^2 \lesssim \frac{\norm{P_{>A}}_2}{n} + \frac{1}{n^2}$. but by Lemma \ref{A_and_1_over_n}, this is equivalent to $\norm{(P-Q)_{>A}}_2^2 \lesssim \frac{1}{n^2}$.

%If $T_1$ accepts, then by Chebyhev's inequality, this implies that $\norm{(P-Q)_{>A}}_1^2 \lesssim \frac{\norm{(P-Q)_{>A}}_1}{n}$.

\noindent Now consider the event
$\{\psi_1 = 0\} \cap \xi.$ On $\{\psi_1 = 0\}$ we have $|T_1| \leq \uc \sqrt{\frac{\|p\|_1}{n}}$ so that on $\xi$:
\begin{align*}
    &\abs{\mathbb{E}[T_1] }\leq \frac{2}{\sqrt \eta} \sqrt{\mathbb{V}[T_1]} + \uc \sqrt{\frac{\|p\|_1}{n}} \Longrightarrow \left|\norm{q}_1-\norm{p}_1\right| \leq \frac{2}{\sqrt \eta} \sqrt{\frac{\norm{q}_1}{n}} + \uc \sqrt{\frac{\|p\|_1}{n}}\\
    &\\
    \Longrightarrow & \norm{q}_1- \norm{p}_1 \leq \frac{2}{\sqrt \eta}\left[ \sqrt{\frac{\norm{p}_1}{n}} + \sqrt{\frac{\norm{\Delta}_1}{n}}\right] + \frac{4}{\sqrt{\eta}} \sqrt{\frac{\|p\|_1}{n}} \\
    &\\
    \Longrightarrow & \norm{\Delta}_1 - 2\norm{p}_1 \leq \frac{3}{\sqrt \eta} \left(\norm{p}_1 + \frac{1}{n}\right)+\frac{2}{\sqrt \eta}\sqrt{\frac{\norm{\Delta}_1}{n}}\\
    &\\
    \Longrightarrow& \norm{\Delta}_1 - \frac{2}{\sqrt{\eta}} \sqrt{\frac{\norm{\Delta}_1}{n}} \leq \left(2 + \frac{3}{\sqrt{\eta}}\right)\norm{p}_1 + \frac{3}{n\sqrt{\eta}}\\
    &\\
    \Longrightarrow & \left(\sqrt{\norm{\Delta}_1} - \frac{1}{\sqrt{n\eta}}\right)^2 - \frac{1}{n\eta} \leq \left(2 + \frac{3}{\sqrt{\eta}}\right)\norm{p}_1 + \frac{3}{n\sqrt{\eta}}\\
    &\\
    \Longrightarrow & \sqrt{\norm{\Delta}_1} - \frac{1}{\sqrt{n\eta}} \leq \sqrt{2+\frac{3}{\eta}}\sqrt{\norm{p}_1} + \sqrt{\frac{1}{\eta} + \frac{3}{\sqrt{\eta}}}\cdot \frac{1}{\sqrt{n}}\\
    &\\
    \Longrightarrow & \sqrt{\norm{\Delta}_1} \leq C_1\sqrt{\norm{p}_1} + C_2\frac{1}{\sqrt{n}}
\end{align*} which we write, for brevity : 
\begin{equation}\label{psi1_and_xi}
    \norm{\Delta}_1 \lesssim \norm{p}_1 + \frac{1}{n}
\end{equation}

\hfill


We now set $\alpha = \frac{1}{t-1}$ and $\beta = \frac{1}{2-t}$, satisfying $\frac{1}{\alpha} + \frac{1}{\beta} = 1$. On $\{\psi_2 = 0\} \cap\{\psi_1 = 0\} \cap \xi,$ Hölder's inequality yields:
\begin{align*}
    \sum_{i > A} \abs{p_i - q_i}^t & = \sum_{i > A} \abs{p_i - q_i}^{2(t-1) + (2-t)} \leq \left(\sum_{i > A} \abs{p_i - q_i}^{2(t-1) \alpha }\right)^\frac{1}{\alpha} \left(\sum_{i > A} \abs{p_i - q_i}^{\beta(2-t)}\right)^\frac{1}{\beta}\\
    & = \left(\sum_{i > A} \abs{p_i - q_i}^2 \right)^{t-1} \left(\sum_{i > A} \abs{p_i - q_i}\right)^{2-t}\\
    & \lesssim \left( \frac{1}{n^2}\right)^{t-1} \left(\norm{p_{>A}}_1 +\frac{1}{n} \right)^{2-t} \text{ using }\eqref{psi2_and_xi} ,\eqref{psi1_and_xi} \\
    &\lesssim \frac{\norm{p_{>A}}_1^{2-t}}{n^{2(t-1)}} + \asymp \frac{1}{n^t}\lesssim \rho^t,
\end{align*} %\al{A preciser. Est ce que $\rho$ est defini?}

Therefore, on $ \{\psi_2 = 0\} \cap\{\psi_1 = 0\} \cap \xi,$ we cannot have
$$\norm{\Delta_{>A}}_t^t  \gtrsim \rho^t,$$
and so our result is proven.



####################################
Ancien test $\psi_2$

We first define the $\chi_2$-related test statistic on the tail coefficients, i.e.~those with index larger than $A$ 
$$T_{2} = \sum_{i > A}  \left(\frac{S_i}{k} - p_i \right)\left(\frac{S'_i}{k} - p_i \right),$$
and the associated test statistic
$$\psi_{2} = \mathbf 1\{|T_2| >  \frac{\uc}{n} \norm{p_{>A}}_2 \},$$


##################################
Ancien blabla sur $\|\cdot\|_2$:

In the special case of the $\|\cdot\|_2$, the test $\psi_2$ actually has the same expression as the bulk test, except that it is applied on the tail coefficients. Indeed, for $t=2$, we have $b=0$: In words, we do not need to renormalize the bulk test, which yields that the bulk and tail test $\psi_2$ have the same expressions. We therefore only need one test, based on the following statistic 
$$ \sum_{j=1}^N \left(\frac{S_j}{n} - p_j\right)\left(\frac{S'_j}{n} - p_j\right)$$
and do not even need to split the distribution into bulk and tail.

##################################
Ancien Poissonization trick

associated to the family of observations $Z_1, \dots, Z_{n'} \overset{iid}{\sim} \mathcal{M}(\frac{\bar q}{\lambda})$. 

\begin{equation}\label{testing_pb_mult}
    H_0^{(Mult)}: \frac{\bar q}{\lambda}= \frac{\bar p}{\lambda} ~~\text{ vs }~~ H_1^{(Mult)}: \left\|\frac{\bar p}{\lambda}-\frac{\bar q}{\lambda}\right\|_{\mathcal{M},t} \geq ~~ \rho_{Mult}^*(n',\frac{\bar p}{\lambda})
\end{equation}


We define $\rho_{Bin},\; \rho_{Poi},\;\rho_{Mult}$ as the minimax separation radii for this testing problems in the binomial, Poisson and multinomial cases respectively, and we show that  $\rho_{Bin}\; \asymp \; \rho_{Poi}\; \asymp \;\rho_{Mult}$.\\




\al{
Plutot:

\begin{equation*}
    H_0: \frac{q}{\sum_i q_i}=p \;\;\;\;\; \text{ v.s. }\;\;\;\;\; H_1: \norm{p-\frac{q}{\sum_i q_i}}_t \geq \rho.
\end{equation*}
Et il faut expliquer pourquoi la borne inf dit des choses sur ce probleme... en effet dans la borne inf tu peux montrer que vu nos priors, avec proba plus grande que $1/2$
$$\|p - \frac{q}{\sum_i q_i}\|_t \geq \|p^{-\max} - q^{-\max}\|_t +c/n.$$
}



\al{Il y a pas mal de petits problemes techniques ici. Je pense que il faut ajuster les inequalite qui vont plutot etre du type
$$ c_{BP}\;\rho_{Bin}(n,p) \leq \rho_{Poi}(n,p,\eta) \leq C_{BP}\;\rho_{Bin}(cn,p, \eta+u),$$
car on va devoir adapter la sample size dans un des deux problemes, ainsi que la proba davoir des echantillons.
}

###########################
Poissonization trick Poi vers Mult

\al{
We now show that $\rho_{Poi}(n,p) \lesssim \rho_{Mult}(n,p)$ when $\sum p_i = 1$. Suppose we observe 
$$ \begin{pmatrix}Y_1 \\ \vdots \\ Y_d\end{pmatrix} \sim \begin{pmatrix} Poi(n q_1) \\ \vdots \\ Poi(n q_d)\end{pmatrix}$$with mutually independent entries, with \textit{a priori} $\sum_{j=1}^d q_j \neq 1$. 


Assume that there exist two absolute constants $c,C$ such that
$c \leq \sum_{j=1}^d q_j \leq C$. Consider the set of vectors $\tilde Z$ of dimension $\tilde n = \sum_i Y_i$ such that its elements are in $\{1, \ldots, d\}$ and such that for any $i$ we have $\sum_j \mathbf 1\{\tilde Z_j = i\} = Y_i$. Consider a $\tilde Z$ in this set taken uniformly at random. By the Poissonisation trick, we know that conditional on $\tilde n$, we have that the coordinates of $\tilde Z$ are independent $\mathcal M(\frac{q}{\sum_i q_i})$.

We then take the $cn/2$ first elements of this vector. There exists a universal constant $c'$ such that with probability $1 - \exp(-c'cn)$, we have $\tilde n \geq nc/2$ so that it is possible to do that on this event. This implies that
$$\rho_{Poi}(n,p,\eta) \lesssim \rho_{Mult}(cn/2,p, \eta + \exp(-c'cn)).$$

}

%\ju{
We still suppose we are given
$$ \begin{pmatrix} Y_1 \\ \vdots \\ Y_d\end{pmatrix} \sim \begin{pmatrix} Poi(nq_1)\\ \vdots \\ Poi(nq_d) \end{pmatrix}$$ where $q=(q_1, \dots, q_d)$ has entries not necessarily summing to $1$.


We consider $(p_1\geq \cdots \geq p_d)$ a vector with positive entries, which do not necessarily sum to $1$. We consider the testing problem \eqref{testing_pb_poisson}.

Let $p_0 \geq p_1$ be arbitrary and define
\begin{equation}\label{def_bar_p}
    \bar p = (p_0, \cdots, p_d) ~~ \text{ and } ~~ \lambda = \sum_{j=0}^d p_j.
\end{equation}\\


The goal is to prove that, for $\lambda$ large enough:
$$ \rho^*_{Poi}(n,p) \lesssim \lambda\rho^*_{Mult}(n\lambda,\bar p/\lambda)$$


\al{Du coup c'est quoi le probleme multinomial de base? Ie on veut quand meme prouver que pour tout $p$ qui somme a 1 on a
$$ \rho_{Poi}(n,p) \lesssim \rho_{Mult}(n,p).$$
Comment on passe de 
$$ \rho_{Poi}(n,p) \lesssim \lambda\rho_{Mult}(n\lambda,\bar p/\lambda),$$
a
$$ \rho_{Poi}(n,p) \lesssim \rho_{Mult}(n,p)$$
dans le cas d'un $p$ qui somme a 1? Et par ailleurs, qu'est ce que tu testes exactement? Le probleme renormalise ou pas?
}

\ju{Tu as raison ce n'était pas clair du tout ! J'ai défini proprement les problèmes poisson et multinomial au-dessus. \\

Pour le problème poisson, on ne veut pas prouver que pour tout $p$ qui somme a 1 on a $ \rho_{Poi}(n,p) \lesssim \rho_{Mult}(n,p)$ En poisson on n'a jamais besoin que le vecteur se somme à 1 et pour les multinomiales, la clé c'est que la shape constraint n'est pas une vraie contrainte: on peut carrément oublier la première coordonnée puisqu'elle se déduit de toutes les autres, donc toute l'information est contenue dans les $d-1$ dernières coordonnées. La seule contrainte d'information est donc que la somme des $d-1$ dernières coordonnées soit comprise entre $0$ et $1$, c'est-à-dire rien comme contrainte, vu l'homogénéité entre $n$ et $p$. Ca veut dire que quand on réduit le vecteur de poisson pour le transformer en multinomiales, il suffit juste de faire en sorte que les $d-1$ dernières coordonnées du vecteur multinomial construit soient un "modèle réduit" du vecteur initial de poisson (que ce soit pour $p$ ou pour $q$). (En fait depuis le début on dit "projeter" mais il vaudrait mieux dire "réduire").\\

Pour ta deuxième question: supposons qu'on ait montré $$ \rho_{Poi}(n,p) \lesssim \lambda\rho_{Mult}(n\lambda,\bar p/\lambda).$$ Attention à droite c'est $\bar p$ et pas $p$ et c'est très important ! De plus on a aussi montré juste avant que lorsque $p'$ se somme à $1$, on a $$\rho_{Mult}(n',p') \asymp \rho_{Poi}(n',p'^{ \; -\max})$$ Pareil, attention c'est $p'^{ \; -\max}$ et pas $p'$. La deuxième relation donne:
$$ \rho_{Mult}(n\lambda,\bar p/\lambda) \asymp \rho_{Poi}(n\lambda, p/\lambda) $$ car $\bar p ^{\; -\max} = p$ donc vu la première relation:
$$ \rho_{Poi}(n,p) \lesssim \lambda \rho_{Mult}(n\lambda,\bar p/\lambda) \asymp \rho_{Poi}(n,p) $$
Ca c'est le bon résultat puisqu'il permet bien de déduire le rate multinomial du rate poisson.}\\


\textbf{\textit{Wlog}, we can assume that} $\sum_{j=1}^d q_j \leq C \sum_{j=1}^d p_j$ for $C$ large enough depending on $p$. Indeed otherwise, we can detect using the first order moment. \\




\noindent Now, we set $$p_0 = \lambda - \sum_{j=1}^d p_j$$ for $\lambda = 1000\; nC\sum_{j=1}^d p_j \left(\sum_{j=1}^d p_j + \frac{1}{n}\right)$. The parameter $\lambda$ is chosen such that $$TV(Poi(n\lambda), Poi(n\lambda - C \sum_{j=1}^d p_j)) \ll \eta$$ [How to tune the constant 1000 ?]

\hfill


Our aim is to prove that 
$$ \rho_{Poi}(n,p) \lesssim \lambda\; \rho_{Mult}(n\lambda,\bar p/\lambda).$$


Therefore, let us assume that the parameter $q$ of the \textbf{Poisson} testing problem is separated away from $p$ as: $$ \|q-p\|_t \gtrsim \lambda \; \rho_{Mult}(n\lambda,\bar p/\lambda)$$ and let us exhibit a test rejecting the null with probability $1 - \frac{\eta}{4}$, with type-I error less that $\frac{\eta}{4}$.\\

\hfill

Consider the following procedure:

\noindent Let $\psi_{Mult}$ be a test well-suited (i.e. with $R(\psi_{Mult}) \leq \eta$) for the \textbf{multinomial} testing problem \eqref{testing_pb_mult} associated with $n' = n\lambda$.

The procedure we propose is as follows: We draw $Y_0 \sim Poi(n\lambda - n\sum_{j=1}^d p_j)$ independently from $Y$. The sample $(Y_0, \cdots, Y_d)$ is indistinguishable from any sample drawn from: $$\left(Poi(n\lambda - n\sum_{j=1}^d q_j), Poi(nq_1), \cdots, Poi(nq_d)\right)$$ by the definition of $\lambda$. Indeed, \ju{(par encadrement)}: we have $0 \leq \sum_j q_j \leq C \sum_j p_j$ and $Poi(n\lambda - 0)$ is indistinguishable from $Poi(n \lambda - C\sum_j p_j)$. Introduce the random function $\widetilde \phi$ performing the ``depoissonization'', i.e. such that, when given $n'$ (not necessarily in $\mathbb{N}$) and a family of random variables 
$$ \begin{pmatrix}y_0\\ \vdots \\ y_d\end{pmatrix} \sim \begin{pmatrix} Poi(n' r_0)\\ \vdots \\ Poi(n'r_d)\end{pmatrix}$$
with $\sum_{j=0}^d r_j = 1$, it decomposes $(y_i)_i$ into $z_1, \cdots, z_{\widetilde n} \overset{iid}{\sim} \mathcal{M}(r_0, \cdots, r_d)$ where $\widetilde n \sim Poi(n')$:

$$ \widetilde \phi(n', y_0, \cdots, y_d) = z_1, \cdots, z_{\widetilde n} \overset{iid}{\sim} \mathcal{M}(r_0, \cdots, r_d) ~~~~ \text{with $\widetilde n \sim Poi(n')$} $$ 

\hfill

\textbf{The testing procedure we propose is:}
\begin{equation}\label{poisson_to_mult_procedure}
    \psi_{Mult} \circ \widetilde \phi (n\lambda, Y_0, \cdots, Y_d) ~~~~ \text{ where } Y_0 \sim Poi(n\lambda - \sum_{j=1}^d p_j) \text{ independent of }Y.
\end{equation}
We now study its type-I and II errors.

\hfill

\textbf{Under the null}: Suppose $q = p$ in the \textbf{Poisson} setting. Then we have 
$$\begin{pmatrix}Y_0\\ \vdots \\ Y_d\end{pmatrix} \sim \begin{pmatrix}Poi(n\lambda - \sum_{j=1}^d p_j) \\ Poi(np_1)\\ \vdots \\ Poi(np_d)\end{pmatrix}$$
hence we can define:
$$Z_1, \cdots, Z_{\widetilde n} := \widetilde \phi(n\lambda, Y_0, \cdots, Y_d) \overset{iid}{\sim} \mathcal{M}\left(\frac{\bar{p}}{\lambda}\right)$$ where $\widetilde n \sim Poi(n\lambda)$. In words, our procedure gives us iid samples drawn from the null hypothesis of the \textbf{multinomial} testing problem. Therefore, by definition, $\psi_{Mult}(Z_1, \cdots, Z_{\widetilde n}) = 0$ with high probability.

\hfill


\textbf{Under the alternative}:

Here,  we suppose that \textbf{in the Poisson testing problem}, we have:
\begin{equation}\label{sep_poi_mult}
     \|p-q\|_t \gtrsim \lambda\; \rho_{Mult}(n\lambda,\bar p/\lambda),
\end{equation}
We will prove that under this assumption the procedure \eqref{poisson_to_mult_procedure} will reject $H_0$ \textit{whp}, yielding $\rho_{Poi}(n,p) \lesssim \lambda \; \rho_{Mult}(n\lambda, \bar p/\lambda)$. Now, let us call $\bar q = (n\lambda - \sum_{j=1}^d q_j, \; q_1, \cdots, q_d)$ and let $\widetilde n \sim Poi(n \lambda)$. Note that \eqref{sep_poi_mult} rewrites equivalently, in terms of the multinomial norm: 
\begin{equation}\label{sep_mult}
    \left\|\frac{\bar{p} - \bar{q} }{\lambda}\right\|_{\mathcal{M},t} \geq \rho_{Mult}(n\lambda, \bar{p}/\lambda)
\end{equation}
 since the multinomial norm does not take the first coordinate into account.\\

Consider $$Z_1, \cdots, Z_{\widetilde n} = \widetilde \phi\left(n\lambda, Y_0, \cdots, Y_d \right).$$

The law of $Z_1, \cdots, Z_{\widetilde n}$ \textit{is not} $\mathcal{M}\left(\frac{\bar{q}}{\lambda}\right)$. However, the true law of such a sample is indistinguishable from $\mathcal{M}\left(\frac{\bar{q}}{\lambda}\right)^{\otimes \widetilde n}$, otherwise it would be possible to distinguish between $Poi(n\lambda)$ and $Poi(n\lambda - C\sum_{j=1}^d p_j)$ which is excluded by the very choice of $\lambda$. [C'est ce point que j'ai du mal à rédiger]. 

Now $\bar{p}/\lambda$ is a probability vector, and we have a sample $Z_1, \cdots, Z_{\widetilde n}$ with a law indistinguishable from $\mathcal{M}(\frac{\bar q}{\lambda})^{\otimes \widetilde n}$. By \eqref{sep_mult} and the definition of $\psi_{Mult}$, it holds that $\psi_{Mult}(Z_1, \cdots, Z_{\widetilde n}) = 1$ with high probability.\\

\hfill\break


################################

Blabla sur les constantes indep de d


\al{Je ne sais pas si ca vaut le coup de garder ce dernier paragraphe...} Since for $n$ large enough the tail term $\frac{\|p_{>A}\|_1^{(2-t)/t}}{n^{(2t-2)/t}}$ is exactly zero, one could wonder why it should be included in the minimax separation rate, and why we do not define a large constant $C>0$ such that for all $p$ we had $ \sqrt{ \frac{\|p_{\leq I}\|_r}{n}} + \frac{\|p_{>A}\|_1^{(2-t)/t}}{n^{(2t-2)/t}} + \frac{1}{n} \leq C\big(\sqrt{ \frac{\|p_{\leq I}\|_r}{n}} + \frac{1}{n}\big)$. The reason is that such a constant would depend on $N$ (the dimension of the problem), whereas we allow the absolute constants to depend only on $\eta$.



################################

Anciens bouts de la discussion

\subsection{Relation with the identity testing problem for multinomials}\label{ss:mult}

\al{this should be in one single item}

%\al{En fait vu que on peut pas direct transformer les resultats de l'un en resultats de l'autre, je pense que c'est plus judicieux de pas dire que les resultats s'appliquent aux multinomiales, mais juste que les settings sont proches mais pas tout a fait les meme... C'est mieux pour faire ressortir la contribution.}


A related problem is the identity testing problem in multinomials as in~\cite{Valiant, Diakonikolas}.

% This is true for the following reason. 



A multinomial distribution can be represented as a vector of probability $\bar q$ of dimension $\bar N$ - with positive entries adding up to $1$. The problem of testing identity to a given multinomial distribution characterised by a vector of probabilities $\bar p$, is the problem of testing, given $n$ data coming from an unknown multinomial distribution characterised by a probability vector $\bar q$, whether $\bar p = \bar q$



\al{A partir de la il faut vraiment reecrire. Il y a trop de choses qui ne sont pas definies (optimal sample complexity...) et qui sont ecrites de facon vraiment imprecises.}

equivalent to testing whether a multinomial distribution represented by a vector $\bar p$ is the same as a given known multinomial distribution represented by a vector $\bar q$. Vector $\bar p$ is unknown but $M$ observations of the multinomial distributions are given, and the plug-in estimator of $\bar p$ based on this sample is denoted by $\hat p$. It is a sufficient statistic of the data for the parameter $\bar q$.

\cite{Valiant} proves the following bounds to characterize the optimal sample complexity $n^*$ when given a fixed $\epsilon$:

$$ \frac{1}{\epsilon} + \frac{\norm{p_{-\epsilon}^{-max}}_{2/3}}{\epsilon} \;\;\lesssim\;\; n^* \;\;\lesssim\;\;\frac{1}{\epsilon} + \frac{\norm{p_{-\epsilon/16}^{-max}}_{2/3}}{\epsilon}$$

In the above bound, $p = (p_1, \cdots, p_N)$ where $p_1 \geq \cdots \geq p_N \geq 0$ and $\sum_{i=1}^n p_i = 1$. For $\alpha > 0$, let $J$ be the smallest index such that $\sum_{i>J} p_i \leq \alpha$. The notation: $\norm{P_{-\alpha}^{-max}}_1$ denotes $\sum_{i=2}^J p_i$.

We show here that these bounds do not match in general. Let $1> \epsilon >0$, let $N>0$ an integer and
$$ p = (1-\epsilon, \frac{\epsilon}{16N}, \cdots, \frac{\epsilon}{16N}) \;\;\;\;\; \text{ so that } \;\;\;\; \norm{p}_1 = 1$$


Then, $\norm{p_{-\epsilon}^{-max}}_{2/3} = 0 \;\;$ and $\;\;\norm{p_{-\epsilon/16}^{-max}}_{2/3} = \left[15N \left(\frac{\epsilon}{16N} \right)^\frac{2}{3} \right]^\frac{3}{2} \asymp \epsilon\sqrt{N}$ so that:\\

$$\frac{1}{\epsilon} + \frac{\norm{p_{-\epsilon}^{-max}}_{2/3}}{\epsilon} = \frac{1}{\epsilon}$$

and 
$$\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\frac{1}{\epsilon} + \frac{\norm{p_{-\epsilon/16}^{-max}}_{2/3}}{\epsilon} = \frac{1+\sqrt{N}}{\epsilon} \gg \frac{1}{\epsilon}$$

for $N \gg 1 $, proving that the bounds do not match.\\

In the present work, we identify matching upper and lower bounds for the same identity testing problem, transposed in the graph case. We conjecture that these results can be transferred to the multinomial setting, using a Poissonization trick.

\hfill \break

Note that \textit{unconditional on the other elements of $\hat p$}, the random variable $n\hat p_i$ follows a Binomial distribution of parameter $(n,\bar p_i)$, and the $\hat p_i$ are correlated.


If we re-index the entries of our adjacency matrix $P$ with a single index $(p'_i)_{i\leq N}$, our setting is equivalent to having $N$ independent Bernoulli distributions with parameters $(n, p'_i)$. Therefore it is clear that our problem is closely related to the identity testing problem for multinomials. 

However, there are two main differences:
\begin{itemize}
    \item We do note impose that $\sum_i p'_i = 1$, which somewhat changes the geometry of the problem. This is particularly true \textit{in the case of the test in Frobenius norm} where the results are trivial whenever $\sum_i p'_i= 1$, as $\epsilon^*$ is then always of order $\frac{1}{n}$ \textit{independently on $Q$}.
    \item The dependence between the $\hat p_i$ in the multinomial setting is also a difference. Because of the Poissonisation trick, see e.g.~\cite{Valiant}, it is expected that the information contained in $\hat p$ is essentially equivalent (up to a multiplicative absolute constant) to the information contained in $\bar N$ independent Poisson distribution with parameter $n\bar p_i$. Again, this is not very different from a Binomial with parameters $(n,\bar p_i)$, at least in terms of information. 
\end{itemize}


%
%\al{Est ce que on a une ref pour tester des multinomiales en Frobenius??}

%\break


%And so our upper and lower bounds would apply in this setting, as we operate 

\hfill


\subsection{Comparison with existing literature}\label{ss:testgraph}




\al{Il faut commencer a comparer avec les resultats one sample. Je ne suis pas sure que ce soit pertinent d'analyser si en detail le two sample test.}

An advantage of our contribution lies in the fact that knowing the minimax separation radius $\epsilon^*(P)$ for all $P$ proves very useful to analyse the two sample testing problem. Given $n$ iid observations $G_1, \cdots, G_n$ drawn from $P$ and $n$ iid observations $H_1, \cdots, H_n$ drawn from $Q$, where both $P$ and $Q$ are unknown, the two sample testing problem is defined as: 
$$ \mathcal{H}_0 : P=Q \;\;\;\;\;\;  \text{ vs }\;\;\;\;\;\; \mathcal{H}_1 : d(P,Q) \geq \epsilon.$$

In other words, we observe two populations of graphs and we want to test whether or not they are generated from the same distribution. This is the problem addressed in~\cite{Alex}. This problem is very related to the present one: In this setting, $P$ is also unknown and observed only through noisy samples. \cite{Alex} consider the class $\mathcal G_\delta$ of sparse graphs, namely $\norm{P}_\infty \leq \delta$ and $\norm{Q}_\infty \leq \delta$. They investigate \textit{uniformly over this class} the minimax separation radius $\epsilon^*$ needed to distinguish $P=Q$ from $d(P,Q) \geq \epsilon^*$, as a function of $n,\delta,\eta$ and for different notions of distances $d$.

In general, the minimax separation radius in the two sample case, with such a sparsity constraint, corresponds to the worst case of the radius in the goodness-of-fit problem over the sparsity class. Obviously, since both $P$ and $Q$ are unknown, the separation radius in the two sample case is necessarily larger. However, to our knowledge, no general theorem allows to transfer directly the results in the goodness-of-fit setting to the two sample case. From this point of view, our results give a lower bound for the two sample setting in terms of the distances $d(P,Q) = \norm{P-Q}_1$ and $d(P,Q) = \norm{P-Q}_2$. 

\cite{Alex} precisely analyse the minimax separation radius for $\norm{P-Q}_2$ and get that, in this case:
\begin{equation}\label{etoile}
 \rho^*_\text{2 sample}  \asymp \sqrt{\frac{m\delta}{n}} \wedge m\delta
 \end{equation}

We recover this result with  Theorem~\ref{Rate}, by taking the worst case over $\mathcal G_\delta$ which amounts to putting all entries of $Q$ to $\delta$.

Therefore, the results in \cite{Alex} \textit{do not depend on $Q$}, i.e. they are not local, but global over the class of sparse graphs to which the graphs corresponding to $(P,Q)$ belong. Note that our results are much more refined, since we characterize the minimax separation radius in the identity testing problem \textit{for all distributions} $Q$, and not just in the worst case of $\mathcal G_\delta$, which only corresponds to the direction $\delta \mathbb{1} \mathbb{1}^T$, where $\mathbb{1}$ is the vector of $\mathbb{R}^m$ with all entries equal to 1.

Investigating the two sample setting in terms of the $l^1$ distance could be an interesting direction for future work \al{This is already done, up to log terms}, all the more since \cite{Alex}'s main conclusion precisely states that the two sample testing problem with sparsity constraints might be feasible or not, depending on what notion of distance is chosen to define the alternative. Moreover, different notions of sparsity are analysed, like constraints on the average degree of the graph, which proves very useful to analyse real-life graphs like social networks, in which no individual can have too many neighbors. Therefore, our very general results could be applied to more realistic modelling problems, in which the combinatorial structure of the graphs, like sparsity, comes into play.

Other papers that consider testing problems in graphs are quite different from our work - e.g.~testing for the presence of communities as in~\cite{Gao_Lafferty} and~\cite{Lei}, or~\cite{Bubeck}, or considering test  statistics on specific features of the graphs as in~\cite{Alex2}, ~\cite{Tang}. A more related stream of literature can be found in the different setting of identity testing for multinomial distributions, see below.

%Since we are interested in local results in this paper, namely minimax results that depend on $Q$, we cannot deduce our rates from this paper. However, their minimax rate for testing in Frobenius norm is of order 

%What we can nevertheless deduce from 

\hfill

\al{Euh la je suis pas trop sure de suivre... Tu veux pas plutot dire

$$ \rho^*(p,n) \underset{n \to \infty}{\asymp} \begin{cases} \sqrt{ \frac{\|p^{-\max}\|_r}{n}} + \frac{1}{n} \leq \frac{1}{N^{(r-1)/(2r)}\sqrt{n}} & \text{ in the multinomial case} \\ ~~~\sqrt{ \frac{\|p\|_r}{n}} ~~~ + \frac{1}{n} \leq \frac{N^{1/(2r)}}{\sqrt{n}} &\text{ in the binomial or Poisson case}.\end{cases}$$


}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Matching bounds Valiant

Let $\rho_{L}$ and $\rho_{U}$ be the lower and upper bounds identified in~\cite{valiant2017automatic}. The quantities $\rho_{L}$ and $\rho_{U}$ are defined implicitly through the following two fixed-point equations
$$ \rho_{L}  = C \sqrt{\frac{\big\|p^{-\max}_{-\rho_L}\big\|_{2/3}}{n}} + \frac{C}{n},$$
$$ \rho_{U}  = c \sqrt{\frac{\big\|p^{-\max}_{-\frac{1}{16}\rho_U}\big\|_{2/3}}{n}} + \frac{c}{n}.$$
This rewriting exactly corresponds to the bounds proposed in~\cite{balakrishnan2019hypothesis}.
Let $\alpha \in [0,1]$ and let $J$ be the index such that if
$\rho = C \sqrt{\frac{\big\|p^{-\max}_{-\alpha\rho}\big\|_{2/3}}{n}} + \frac{C}{n},$ then $p^{-\max}_{-\alpha\rho} = p^{-\max}_{\leq J}$. In our example we have $J = 1+\lceil(1-\alpha)(N-1)\rceil $, hence
\begin{align*}
    \rho = C \sqrt{\frac{(J-1)^{3/2}}{n}\frac{\rho}{N}} + \frac{C}{n} \Longrightarrow \rho \asymp (1-\alpha)^\frac{3}{4}\frac{\sqrt{N}}{n} + \frac{1}{n}.
\end{align*}
Therefore, we get $\rho_U \asymp \frac{\sqrt{N}}{n}$ and $\rho_L \asymp \frac{1}{n}$ for $\sqrt{N} \geq n$, proving that even when translated in terms of separation radius, the bounds identified in~\cite{valiant2017automatic} and in~\cite{balakrishnan2019hypothesis} do not match. \\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Non matching bounds valiant
We now justify that, when translated in terms of separation radius, the upper and lower bounds also do not match, whereas ours do.

Let $\rho_{L}$ and $\rho_{U}$ be the lower and upper bounds which can be derived from~\cite{valiant2017automatic}. The quantities $\rho_{L}$ and $\rho_{U}$ are defined implicitly through the following two fixed-point equations
$$ \rho_{L}  = C \sqrt{\frac{\big\|p^{-\max}_{-\rho_L}\big\|_{2/3}}{n}} + \frac{C}{n},$$
$$ \rho_{U}  = c \sqrt{\frac{\big\|p^{-\max}_{-\frac{1}{16}\rho_U}\big\|_{2/3}}{n}} + \frac{c}{n}.$$
This rewriting exactly corresponds to the bounds proposed in~\cite{balakrishnan2019hypothesis}. Now, consider \textit{any} null distribution $p$ such that $p_{-\rho_L} \neq p$. Two find an example of non matching upper and lower bounds, it suffices to modify the null distribution $p$ as follows. Denote by $J$ the cut-off index such that $p_{-\rho_L} = p_{\leq J}$.
Define the distribution $\widetilde p$ such that $\forall j \leq J: \widetilde p_j = p_j$ and spread the remaining mass on an arbitrary large finite set: namely, for $d \in \mathbb N$ sufficiently larger than $N$, set $\widetilde p_j = \frac{\|p_{>J}\|_1}{d-J}$ for all $j = J+1, \dots, d$. 
By definition of $\widetilde p$, we have $\rho_L(\widetilde p) = \rho_L(p)$. As for the upper bound

We now prove that our bounds do match in this example. Let us solve
\begin{align*}
    \rho = C \left(\sqrt{\frac{\big\|p^{-\max}_{\leq I}\big\|_{2/3}}{n}} \lor \|p_{>I}\|_1 \lor \frac{1}{n}\right),
\end{align*}
where $I$ is the smallest integer such that $n^2\|p_{>I}\|_2^2 \leq \cI$. Note that recalling the expression of $p$ from~\eqref{ex:example_p}, the latter condition implies that $I \geq \frac{N}{2}$ if $N^2 \geq n$.
\begin{enumerate}
    \item First case: if $\rho = C\sqrt{\frac{\big\|p^{-\max}_{\leq I}\big\|_{2/3}}{n}}$, then 
\end{enumerate}

\hfill


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Preuve valiant pas tight

We show here that the upper and lower bounds do not match up to universal constants in some cases. Let $1> \epsilon >0$, let $N>0$ an integer and
\begin{equation}\label{ex:example_p}
    p = (1-\epsilon, \frac{\epsilon}{N-1}, \cdots, \frac{\epsilon}{N-1}) \;\;\;\;\; \text{ so that } \;\;\;\; \left\|p\right\|_1 = 1.
\end{equation}
 

Then, $\norm{p_{-\epsilon}^{-\max}}_{2/3} = 0 \;\;$ and $\;\;\norm{p_{-\epsilon/16}^{-\max}}_{2/3} \asymp \left[\frac{15(N-1)}{16} \left(\frac{\epsilon}{16(N-1)} \right)^\frac{2}{3} \right]^\frac{3}{2} \asymp \epsilon\sqrt{N}$ so that:
$$\frac{1}{\epsilon} + \frac{\norm{p_{-\epsilon}^{-\max}}_{2/3}}{\epsilon} = \frac{1}{\epsilon}$$

and 
$$\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\frac{1}{\epsilon} + \frac{\norm{p_{-\epsilon/16}^{-\max}}_{2/3}}{\epsilon} = \frac{1+\sqrt{N}}{\epsilon} \gg \frac{1}{\epsilon}$$

for $N \gg 1 $, proving that the bounds do not match.\\

s







